BookSum: A Collection of Datasets for Long-form Narrative Summarization

The majority of available text summarization datasets include short-form source documents that lack long-range causal and temporal dependencies, and often contain strong layout and stylistic biases. While relevant, such datasets will offer limited challenges for future generations of text summarization systems. We address these issues by introducing BookSum, a collection of datasets for long-form narrative summarization. Our dataset covers source documents from the literature domain, such as novels, plays and stories, and includes highly abstractive, human written summaries on three levels of granularity of increasing difficulty: paragraph-, chapter-, and book-level. The domain and structure of our dataset poses a unique set of challenges for summarization systems, which include: processing very long documents, non-trivial causal and temporal dependencies, and rich discourse structures. To facilitate future work, we trained and evaluated multiple extractive and abstractive summarization models as baselines for our dataset.

==> 8-response.tex <==
\section*{BookSum: A Collection of Datasets for Long-form Narrative Summarization}
\subsection*{Author Response}
In response to the ARR meta-review, we kindly ask you to consider the following:


For data that is no longer protected by copyright law, we understand the use described within the paper is legally permissible.
%
For data that is subject to copyright (book summaries), we understand that such use is allowed under U.S. copyright law's fair use provision.
%
Depending on how others use this data, the purpose of their use, the jurisdiction they are in, and other factors considered under copyright law, we understand that the decision on whether a specific use case is fair use involves a legal analysis.
%
As with other text summarization datasets based on Web resources that were previously accepted to *CL venues, it is advisable to obtain legal counsel prior to using such data.

We will also include an extended discussion of the ethical considerations and limitations regarding use of the data in the Limitations section.
%
Following suggestions of the ARR reviewers, we will also add a more detailed description of how data was collected and processed in the camera-ready version of this paper.
%
Alongside this work, we share code resource which allow to reliably recreate the \DatasetName~dataset.

\newpage
\section*{Limitations}
%
\paragraph{Data Collection}
%
Web data is subject to local copyright laws.
%
For data that is no longer protected by copyright law, we understand the use described within the paper is legally permissible.
%
For data that is subject to copyright, we understand that such use is allowed under U.S. copyright law's fair use provision.
%
Depending on how others use this data, the purpose of their use, the jurisdiction they are in, and other factors considered under copyright law, we understand that the decision on whether a specific use case is fair use involves a legal analysis.
%
It is advisable to obtain legal counsel prior to using such data.
%
All data described in this work was collected exclusively for the academic purpose of conducting research.
%
The purpose of using the \DatasetName~data was only for training models and not for public display or any other use.
%
No data was stored upon completion of the research process.

\paragraph{Data Biases}
%
The \DatasetName~dataset contains books written or translated into English.
%
These books are also more than fifty years old and so representative of society in that era.
%
The various pretrained models we evaluated on our dataset carry biases of the data they were pretrained on.
%
However, we did not stress test these models for such ethical biases.
%
We request our users to be aware of these ethical issues in our dataset that might affect their models and evaluations.

\paragraph{Model Evaluation}
%

%
In this work, we have used established metrics, such as ROUGE, as well as recently introduced metrics, such as BERTScore and SummaQA, to evaluate the introduced baseline models.
%
However, such automatic metrics have not been evaluated for use with very long source documents and highly abstractive summaries. 
%
Thus, might not accurately reflect the true performance of the evaluated models.
%
Reliable evaluation of highly abstractive summarization models trained on long source documents is an open problem and an area of active research.
%
Authors using the \DatasetName~data are encouraged to consult appropriate literature whether more robust evaluation methods are available at the time of writing.

\paragraph{Computational Resources}
%
Considering the length of source documents included in the \DatasetName~dataset, training and evaluation of neural models might require substantial computational resources.


==> tables/booksum2.0-rouge-scores.tex <==
\begin{table*}[tb]
    \centering
    \resizebox{\linewidth}{!}{%
    \small
    \begin{tabular}{lrrrrrrrrrrrrrrr} 
    \toprule
    & \multicolumn{6}{c}{\DatasetName-Paragraph} & \multicolumn{6}{c}{\DatasetName-Chapter} & \multicolumn{6}{c}{\DatasetName-Book} \\
    \cmidrule(lr){2-6} 
    \cmidrule(lr){7-11}
    \cmidrule(lr){12-16}
    \textbf{Models} & $\textrm{R-1}_{f_1}$ & $\textrm{R-2}_{f_1}$ & $\textrm{R-L}_{f_1}$ & $\textrm{BS}_{f_1}$ & $\textrm{SQA}_{f_1}$ & $\textrm{FEQA}_{f_1}$ & $\textrm{R-1}_{f_1}$ & $\textrm{R-2}_{f_1}$ & $\textrm{R-L}_{f_1}$ & $\textrm{BS}_{f_1}$ & $\textrm{SQA}_{f_1}$  & $\textrm{FEQA}_{f_1}$ & $\textrm{R-1}_{f_1}$ & $\textrm{R-2}_{f_1}$ & $\textrm{R-L}_{f_1}$ & $\textrm{BS}_{f_1}$ & $\textrm{SQA}_{f_1}$  & $\textrm{FEQA}_{f_1}$\\
    \midrule
    & & \multicolumn{12}{c}{Heuristics} \\
    \midrule
    
    Lead-3 & 18.12 & 3.18 & 12.68 & 
    0.084 & 26.77 & 15.70 & 2.46 & 9.06 & 0.001  & 12.18 & 6.99 & 0.91 & 4.57 & -0.057 & 9.19 \\
    Random Sentences & 17.93 & 3.09 & 12.30 & 0.075  & 10.36 & 13.83 & 1.50 & 7.94 & -0.017 & 8.20 & 5.21 & 0.54 & 3.23 & -0.091 & 7.21 \\
    Extractive Oracle & 27.27 & 6.81 & 20.30 & 0.156  & 19.70 & 42.68 & 9.66 & 21.33 & 0.150 & 13.49 & 46.62 & 9.17 & 18.31 & 0.082 & 21.16 \\
    \midrule
    & & \multicolumn{11}{c}{Extractive Models} \\
    \midrule
    CNN-LSTM  & 16.31 & 2.72 & 12.58 & 0.068 & 15.18 & 32.50 & 5.75  & 13.65  & 0.075 & 11.27 & 35.16 & 5.71 & 13.03 & 0.016 & 21.47   \\
    BertExt & 14.14 & 2.18 & 10.26 & 0.053 & 14.89 & 33.04 & 5.78 & 13.74 & 0.082 & 14.33 & 36.71 & 6.16 & 13.40 & 0.028 & 24.83 \\
    MatchSum & 18.06 & 2.97 & 13.35 & 0.101 & 17.79 & 30.26 & 4.81  & 12.90 & 0.072 & 8.02 & 31.77 & 4.78 & 12.22 & 0.009 & 23.22 \\
    \midrule
    & & \multicolumn{11}{c}{Abstractive Models} \\
    \midrule
    BART~\textsubscript{zero-shot} & 17.39 & 2.21 & 12.93 & 0.121 & 13.58 & 32.15 & 5.54 & 14.27 & 0.089 & 12.59 & 35.38 & 5.38 & 12.95 & 0.022 & 12.97 \\
    T5~\textsubscript{zero-shot} & 19.10 & 3.29 & 13.46 & 0.082 & 20.41 & 31.8 & 5.41 & 13.00 & 0.075 & 20.49 & 35.43 & 5.62 & 12.02 & 0.011 & 22.77 \\
    PEGASUS~\textsubscript{zero-shot} & 13.98 & 1.74 & 10.93 & 0.093 & 10.50 & 28.70 & 4.43 & 13.34 & 0.056 & 9.69 & 32.24 & 4.84 & 12.20 & 0.004 & 10.50 \\
    %$\textrm{Big Bird}_{zero shot}$ & r1 & r2 & rl & bs & sqa & r1 & r2 & rl & bs & sqa & r1 & r2 & rl & bs & sqa \\
    
    \midrule
    BART~\textsubscript{fine-tuned} & 22.08 & 4.82 & 16.89 & 0.187 & 17.31 & 37.09 & 8.23 & 15.37 & 0.139 & 16.98 & 29.97 & 6.02 & 10.97 & 0.036 & 20.46 \\
    T5~\textsubscript{fine-tuned} & 21.01 & 4.74 & 16.83 & 0.198 & 15.80 & 37.38 & 8.42 & 16.77 & 0.150 & 15.40 & 39.46 & 7.69 & 13.77 & 0.060 & 18.33 \\
    PEGASUS~\textsubscript{fine-tuned} & 19.47 & 4.32 & 15.70 & 0.179 & 12.37 & 36.17 & 7.79 & 16.09 & 0.129 & 13.12 & 35.29 & 6.79 & 12.71 & 0.042 & 18.76 \\
    
    & & \multicolumn{11}{c}{Abstractive Models} \\
    \midrule
    BART~\textsubscript{zero-shot} & 17.39 & 2.21 & 12.93 & 0.121 & 13.58 & 32.15 & 5.54 & 14.27 & 0.089 & 12.59 & 35.38 & 5.38 & 12.95 & 0.022 & 12.97 \\
    T5~\textsubscript{zero-shot} & 19.10 & 3.29 & 13.46 & 0.082 & 20.41 & 31.8 & 5.41 & 13.00 & 0.075 & 20.49 & 35.43 & 5.62 & 12.02 & 0.011 & 22.77 \\
    PEGASUS~\textsubscript{zero-shot} & 13.98 & 1.74 & 10.93 & 0.093 & 10.50 & 28.70 & 4.43 & 13.34 & 0.056 & 9.69 & 32.24 & 4.84 & 12.20 & 0.004 & 10.50 \\
    %$\textrm{Big Bird}_{zero shot}$ & r1 & r2 & rl & bs & sqa & r1 & r2 & rl & bs & sqa & r1 & r2 & rl & bs & sqa \\
    
    \midrule
    BART~\textsubscript{fine-tuned} & 22.08 & 4.82 & 16.89 & 0.187 & 17.31 & 37.09 & 8.23 & 15.37 & 0.139 & 16.98 & 29.97 & 6.02 & 10.97 & 0.036 & 20.46 \\
    T5~\textsubscript{fine-tuned} & 21.01 & 4.74 & 16.83 & 0.198 & 15.80 & 37.38 & 8.42 & 16.77 & 0.150 & 15.40 & 39.46 & 7.69 & 13.77 & 0.060 & 18.33 \\
    PEGASUS~\textsubscript{fine-tuned} & 19.47 & 4.32 & 15.70 & 0.179 & 12.37 & 36.17 & 7.79 & 16.09 & 0.129 & 13.12 & 35.29 & 6.79 & 12.71 & 0.042 & 18.76 \\
    %$\textrm{Big Bird}_{fine-tuned}$ & r1 & r2 & rl & bs & sqa & r1 & r2 & rl & bs & sqa & r1 & r2 & rl & bs & sqa \\
    %\midrule
    %\midrule
    %GPT-3 6B & - & - & - & - & - & - & - & - & - & - & 36.78 & 7.22 & 14.83 & 0.1245 & - \\
    %GPT-3 175B & - & - & - & - & - & - & - & - & - & - & 41.50 & 10.46 & 16.87 & 0.1820 & - \\
    %GPT-3 175B (1st tree) & - & - & - & - & - & - & - & - & - & - & 43.19 & 10.63 & 17.10 & 0.1820 & - \\
    
    
    \bottomrule
    \end{tabular}
    }%
    \caption{
    Booksum 2.0 scores for comparison
    % Don't add newlines here.
    }
    \label{tab:booksum2.0-rouge-scores}
\end{table*}




==> tables/summary-example.tex <==
\begin{table*}[th!]
    \centering
    %\resizebox{\linewidth}{!}{%
    \small
    \begin{tabular}{p{\linewidth}} 
    \toprule
    \textbf{Book-level summary of "Gulliver's Travels"} \\
    \midrule
    Lemuel Gulliver is a married surgeon from Nottinghamshire, England, who has a taste for traveling. He heads out on a fateful voyage to the South Seas when he gets caught in a storm and washed up on an island. This island, Lilliput, has a population of tiny people about 6 inches tall. They capture Gulliver as he sleeps and carry him to their capital city, where they keep him chained inside a large abandoned temple outside the city walls. Gulliver becomes a great friend of the Emperor of Lilliput (...) %, who introduces Gulliver to many of their customs. For example, instead of staffing his cabinet with capable administrators, the Emperor chooses guys who perform best at a dangerous kind of rope dancing. The Emperor asks Gulliver to help him in his war against Blefuscu, a similarly tiny kingdom across a channel of water. Gulliver agrees and uses his huge size to capture all of Blefuscu's navy.In spite of the great service that Gulliver has done for the Lilliputians, he has two terrible enemies, who seem to be jealous of his strength and favor with the Emperor: the admiral Skyresh Bolgolam and the treasurer Flimnap. These two men conspire to influence the Emperor to have Gulliver executed. They serve Gulliver with a series of Articles of Impeachment, with the final sentence that Gulliver is going to be blinded. Gulliver is informed of this plot against him by a friend at the Lilliputian court. He manages to escape to the island of Blefuscu. Fortunately for him, a human-sized boat washes ashore on Blefuscu. Gulliver rows to nearby Australia and finds a boat to take him back to England.Gulliver heads out to sea again after a brief stay in England with his family . Once again, a storm blows up, and Gulliver winds up on the island of Brobdingnag. The Brobdingnag are giants 60 feet tall, who treat Gulliver like an attraction at a fair. Gulliver comes to the attention of the Brobdingnagian Queen, who keeps him like a kind of pet. She is amused, because he is so tiny and yet still manages to speak and act like a real person. This Queen employs a young girl, Glumdalclitch, to look after Gulliver and teach him their language. (...)
    \\
    \midrule
    \textbf{Chapter-level summary of "Gulliver's Travels"} \\
    \midrule
    Our hero, Lemuel Gulliver, starts out his adventures with a description of his origins: he's from Nottinghamshire in England, and he has spent several years at college at Cambridge. Sadly, Gulliver's father runs out of money for young Gulliver's education, so he sends Gulliver as an apprentice to Mr. James Bates, a London surgeon. Gulliver also spends a lot of time studying math and navigation, because he wants to travel. Eventually, with the financial help of his uncle, his father, and some other (...) % relatives Gulliver travels to Leyden, where there is a famous university known for its teaching of medicine. After studying at Leyden for a couple of years, Gulliver returns to England, where Mr. Bates gives Gulliver a recommendation to join the crew of the ship the Swallow as a surgeon. Gulliver travels for three years on the Swallow and gets as far as the Levant He comes back to London and settles down to marry Mrs. Mary Burton, who comes with a dowry of 400 pounds - nice for Gulliver! Gulliver's former boss and current patron, Mr. Bates dies a couple of years later, and Gulliver's business starts to go bad. Gulliver decides to go to sea again, traveling this time to the Far East and the West Indies. He spends a lot of time reading while he's at sea; when Gulliver is ashore, he enjoys observing the customs of the people he meets. But even the sea starts to lose its interest for Gulliver, and he decides to head home to London to hang out with his wife. Gulliver moves his business to various parts of London, but he continues to fail at making a living, so he hits the sea once again three years later. He sets sail with Captain William Prichard on the Antelope, heading to the South Seas As you might expect, things go wrong. All of the following happens in one long paragraph:A storm blows up.The ship winds up in the Northwest of "Van Diemen's Land" - what we now call Tasmania, an area in the southeast of Australia. 12 members of the ship's crew die and the rest are weakened by hard work and lack of food. (...)
    \\
    \midrule
    \textbf{Paragraph-level summary of "Gulliver's Travels"} \\
    \midrule
    Our hero, Lemuel Gulliver, starts out his adventures with a description of his origins: he's from Nottinghamshire in England, and he has spent several years at college at Cambridge. Sadly, Gulliver's father runs out of money for young Gulliver's education, so he sends Gulliver as an apprentice to Mr. James Bates, a London surgeon. %Gulliver also spends a lot of time studying math and navigation, because he wants to travel.
    \\
    \bottomrule
    \end{tabular}
    %}%
    \caption{
    Examples of summaries on full-book-, chapter-, and paragraph-levels collected for the same book. 
    %
    }
    \label{tab:summary-examples}
\end{table*}
